GLUS: Global-Local Reasoning Unified into A Single Large Language Model for Video Segmentation

This paper proposes a novel framework utilizing multi-modal large language models (MLLMs) for referring video object segmentation (RefVOS). Previous MLLM-based methods commonly struggle with the dilemma between "Ref" and "VOS": they either specialize in understanding a few key frames (global reasoning) or tracking objects on continuous frames (local reasoning), and rely on external VOS or frame selectors to mitigate the other end of the challenge. However, our framework GLUS shows that global and local consistency can be unified into a single video segmentation MLLM: a set of sparse "context frames" provides global information, while a stream of continuous "query frames" conducts local object tracking. This is further supported by jointly training the MLLM with a pre-trained VOS memory bank to simultaneously digest short-range and long-range temporal information. To improve the information efficiency within the limited context window of MLLMs, we introduce object contrastive learning to distinguish hard false-positive objects and a self-refined framework to identify crucial frames and perform propagation. By collectively integrating these insights, our GLUS delivers a simple yet effective baseline, achieving new state-of-the-art for MLLMs on the MeViS and Ref-Youtube-VOS benchmark. Our project page is at https://glus-video.github.io/.

==> tables/ablation_global_local_segmentor.tex <==
\begin{table}[t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l@{\hspace{8mm}}|c@{\hspace{6mm}}c@{\hspace{6mm}}}
\toprule
 Method & MeViS (valid_u) & RefYoutube \\ 
 \midrule
Single Segmentor (LISA) & 44.8 & 50.2 \\
Global Segmentor (8 frames) & 45.16 & 52.38 \\
Local Segmentor (8 frames) & 49.86 & 54.61 \\
Global-Local Segmentor (4+4 frames) & \textbf{50.19} & \textbf{56.52} \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{
}
\vspace{-4mm}
\label{tab:ablation_global_local_segmentor}
\end{table}

==> tables/ablation_memory_bank.tex <==
\begin{table}[t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l@{\hspace{8mm}}|c@{\hspace{6mm}}c@{\hspace{6mm}}}
\toprule
 Method & MeViS (valid_u) & RefYoutube \\ 
 \midrule
\ourwork (w/o memory bank) & 58.25 & 63.56 \\
\midrule
\ourwork (memory stride 1) & & \\
\ourwork (memory stride 3) & 59.65 & 65.16 \\
\ourwork (memory stride 5) & & \\
\ourwork (memory stride 7) & & \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{
}
\vspace{-4mm}
\label{tab:ablation_memory_bank}
\end{table}
